The ALICE experiment: a journey through QCD

The ALICE experiment was proposed in 1993, to study strongly-interacting matter at extreme energy densities and temperatures. This proposal entailed a comprehensive investigation of nuclear collisions at the LHC. Its physics programme initially focused on the determination of the properties of the quark-gluon plasma (QGP), a deconfined state of quarks and gluons, created in such collisions. The ALICE physics programme has been extended to cover a broader ensemble of observables related to Quantum Chromodynamics (QCD), the theory of strong interactions. The experiment has studied Pb-Pb, Xe-Xe, p-Pb and pp collisions in the multi-TeV centre of mass energy range, during the Run 1-2 data-taking periods at the LHC (2009-2018). The aim of this review is to summarise the key ALICE physics results in this endeavor, and to discuss their implications on the current understanding of the macroscopic and microscopic properties of strongly-interacting matter at the highest temperatures reached in the laboratory. It will review the latest findings on the properties of the QGP created by heavy-ion collisions at LHC energies, and describe the surprising QGP-like effects in pp and p-Pb collisions. Measurements of few-body QCD interactions, and their impact in unraveling the structure of hadrons and hadronic interactions, will be discussed. ALICE results relevant for physics topics outside the realm of QCD will also be touched upon. Finally, prospects for future measurements with the ALICE detector in the context of its planned upgrades will also be briefly described.

==> Chapter3/Chapter3.4/commands.tex <==

\newcommand{\pp}           {pp\xspace}
\newcommand{\ppbar}        {\mbox{$\mathrm {p\overline{p}}$}\xspace}
\newcommand{\XeXe}         {\mbox{Xe--Xe}\xspace}
\newcommand{\PbPb}         {\mbox{Pb--Pb}\xspace}
\newcommand{\pA}           {\mbox{pA}\xspace}
\newcommand{\pPb}          {\mbox{p--Pb}\xspace}
\newcommand{\Pbp}          {\mbox{Pb--p}\xspace}
\newcommand{\AuAu}         {\mbox{Au--Au}\xspace}
\newcommand{\dAu}          {\mbox{d--Au}\xspace}

\newcommand{\s}            {\ensuremath{\sqrt{s}}\xspace}
\newcommand{\snn}          {\ensuremath{\sqrt{s_{\mathrm{NN}}}}\xspace}
\newcommand{\pt}           {\ensuremath{p_{\rm T}}\xspace}
\newcommand{\meanpt}       {$\langle p_{\mathrm{T}}\rangle$\xspace}
\newcommand{\minv}         {\ensuremath{m_{\rm inv.}}\xspace}
\newcommand{\ycms}         {\ensuremath{y_{\rm CMS}}\xspace}
\newcommand{\ylab}         {\ensuremath{y_{\rm lab}}\xspace}
\newcommand{\etarange}[1]  {\mbox{$\left | \eta \right |~<~#1$}}
\newcommand{\yrange}[1]    {\mbox{$\left | y \right |~<~#1$}}
\newcommand{\dndy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\dndeta}       {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}\eta}\xspace}
\newcommand{\avdndeta}     {\ensuremath{\langle\dndeta\rangle}\xspace}
\newcommand{\dNdy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\Npart}        {\ensuremath{N_\mathrm{part}}\xspace}
\newcommand{\Ncoll}        {\ensuremath{N_\mathrm{coll}}\xspace}
\newcommand{\dEdx}         {\ensuremath{\textrm{d}E/\textrm{d}x}\xspace}
\newcommand{\RpPb}         {\ensuremath{R_{\rm pPb}}\xspace}
\newcommand{\mpt}          {\ensuremath{\langle p_{\rm T}\rangle}\xspace}
\newcommand{\mptsquared}   {\ensuremath{\langle p^2_{\rm T}\rangle}\xspace}
\newcommand{\RAA}          {\ensuremath{R_{\rm AA}}\xspace}
\newcommand{\RpA}          {\ensuremath{R_{\rm pA}}\xspace}

\newcommand{\nineH}        {$\sqrt{s}~=~0.9$~Te\kern-.1emV\xspace}
\newcommand{\seven}        {$\sqrt{s}~=~7$~Te\kern-.1emV\xspace}
\newcommand{\twoH}         {$\sqrt{s}~=~0.2$~Te\kern-.1emV\xspace}
\newcommand{\twosevensix}  {$\sqrt{s}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\five}         {$\sqrt{s}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\thirteen}     {$\sqrt{s}~=~13$~Te\kern-.1emV\xspace}
\newcommand{\twosevensixnn}{$\sqrt{s_{\mathrm{NN}}}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\fivenn}       {$\sqrt{s_{\mathrm{NN}}}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\eightnn}       {$\sqrt{s_{\mathrm{NN}}}~=~8.16$~Te\kern-.1emV\xspace}
\newcommand{\LT}           {L{\'e}vy-Tsallis\xspace}
\newcommand{\GeVc}         {Ge\kern-.1emV/$c$\xspace}
\newcommand{\MeVc}         {Me\kern-.1emV/$c$\xspace}
\newcommand{\TeV}          {Te\kern-.1emV\xspace}
\newcommand{\GeV}          {Ge\kern-.1emV\xspace}
\newcommand{\MeV}          {Me\kern-.1emV\xspace}
\newcommand{\GeVmass}      {Ge\kern-.2emV/$c^2$\xspace}
\newcommand{\MeVmass}      {Me\kern-.2emV/$c^2$\xspace}
\newcommand{\lumi}         {\ensuremath{\mathcal{L}}\xspace}

\newcommand{\ITS}          {\rm{ITS}\xspace}
\newcommand{\TOF}          {\rm{TOF}\xspace}
\newcommand{\ZDC}          {\rm{ZDC}\xspace}
\newcommand{\ZDCs}         {\rm{ZDCs}\xspace}
\newcommand{\ZNA}          {\rm{ZNA}\xspace}
\newcommand{\ZNC}          {\rm{ZNC}\xspace}
\newcommand{\SPD}          {\rm{SPD}\xspace}
\newcommand{\SDD}          {\rm{SDD}\xspace}
\newcommand{\SSD}          {\rm{SSD}\xspace}
\newcommand{\TPC}          {\rm{TPC}\xspace}
\newcommand{\TRD}          {\rm{TRD}\xspace}
\newcommand{\VZERO}        {\rm{V0}\xspace}
\newcommand{\VZEROA}       {\rm{V0A}\xspace}
\newcommand{\VZEROC}       {\rm{V0C}\xspace}
\newcommand{\Vdecay} 	   {\ensuremath{V^{0}}\xspace}

\newcommand{\jpsi}         {\ensuremath{\text{J}/\psi}\xspace}
\newcommand{\psiprime}     {\ensuremath{\psi(2\text{S})}\xspace}
\newcommand{\ccbar}        {\ensuremath{\text{c}\overline{\text{c}}}\xspace}
\newcommand{\bbbar}        {\ensuremath{\text{b}\overline{\text{b}}}\xspace}
\newcommand{\ee}           {\ensuremath{\text{e}^{+}\text{e}^{-}}\xspace} 
\newcommand{\mumu}           {\ensuremath{\mu^{+}\mu^{-}}\xspace} 
\newcommand{\pip}          {\ensuremath{\pi^{+}}\xspace}
\newcommand{\pim}          {\ensuremath{\pi^{-}}\xspace}
\newcommand{\kap}          {\ensuremath{\rm{K}^{+}}\xspace}
\newcommand{\kam}          {\ensuremath{\rm{K}^{-}}\xspace}
\newcommand{\pbar}         {\ensuremath{\rm\overline{p}}\xspace}
\newcommand{\kzero}        {\ensuremath{{\rm K}^{0}_{\rm{S}}}\xspace}
\newcommand{\lmb}          {\ensuremath{\Lambda}\xspace}
\newcommand{\almb}         {\ensuremath{\overline{\Lambda}}\xspace}
\newcommand{\Om}           {\ensuremath{\Omega^-}\xspace}
\newcommand{\Mo}           {\ensuremath{\overline{\Omega}^+}\xspace}
\newcommand{\X}            {\ensuremath{\Xi^-}\xspace}
\newcommand{\Ix}           {\ensuremath{\overline{\Xi}^+}\xspace}
\newcommand{\Xis}          {\ensuremath{\Xi^{\pm}}\xspace}
\newcommand{\Oms}          {\ensuremath{\Omega^{\pm}}\xspace}
\newcommand{\degree}       {\ensuremath{^{\rm o}}\xspace}
\newcommand{\upsone}         {\ensuremath{\Upsilon(1\text{S})}\xspace}
\newcommand{\upstwo}         {\ensuremath{\Upsilon(2\text{S})}\xspace}
\newcommand{\upsthree}         {\ensuremath{\Upsilon(3\text{S})}\xspace}
\newcommand{\rmJpsi}    {\mbox{$\mathrm{J\kern-0.05em /\kern-0.05em\psi}$}}
\newcommand{\velip}         {\ensuremath{v_{\rm 2}}\xspace}


\newcommand{\note}[1]{{\color{red}\textbf{#1}}}


==> Chapter3/Chapter3.5/include.tex <==

\newcommand{\CommentBlock}[1]{}

\newcommand{\redtext}[1]{\textcolor{red}{#1}}
\newcommand{\bluetext}[1]{\textcolor{blue}{#1}}
\newcommand{\greentext}[1]{\textcolor{green}{#1}}



\newcommand{\dAu}{d--Au}
\newcommand{\AuAu}{Au--Au}
\newcommand{\PbPb}{Pb--Pb}
\newcommand{\pPb}{p--Pb}
\newcommand{\pbarp}{bar{p}p}
\newcommand{\pp}{pp}
\newcommand{\pA}{p--A}
\newcommand{\aaa}{\ensuremath{A+A}}

\newcommand{\sqrtsNN}{\ensuremath{\sqrt{s_{NN}}}}
\newcommand{\sqrts}{\ensuremath{\sqrt{s}}}

\newcommand{\intlumi}{\ensuremath{L_{\mathrm{int}}}}
\newcommand{\invmub}{\ensuremath{\mu{b}^{-1}}}
\newcommand{\invnb}{{nb}$^{-1}$}
\newcommand{\gev}{\ensuremath{\mathrm{GeV/}c}}

\newcommand{\alphas}{\ensuremath{\alpha_{s}}}


\newcommand{\Nbin}{\ensuremath{N_{bin}}}
\newcommand{\Ncoll}{\ensuremath{N_{coll}}}
\newcommand{\Npart}{\ensuremath{N_{part}}}
\newcommand{\Nbinavg}{\ensuremath{\left<N_{bin}\right>}}

\renewcommand{\Nbinavg}{\ensuremath{\left<N_{bin}\right>}}
\newcommand{\TAA}{\ensuremath{\left<T_{\mathrm{AA}}\right>}}
\newcommand{\TpPb}{\ensuremath{\left<T_{\mathrm{pPb}}\right>}}
\newcommand{\TdAu}{\ensuremath{\left<T_{\mathrm{dAu}}\right>}}
\newcommand{\TpA}{\ensuremath{\left<T_{\mathrm{p}A}\right>}}



\newcommand{\rr}{\ensuremath{R}}
\newcommand{\kT}{\ensuremath{k_\mathrm{T}}}
\newcommand{\antikT}{anti-\ensuremath{k_\mathrm{T}}}

\newcommand{\Ajet}{\ensuremath{A_\mathrm{jet}}}
\newcommand{\rhoA}{\ensuremath{\rho\times\Ajet}}


\newcommand{\pT}{\ensuremath{p_\mathrm{T}}}
\newcommand{\meanpT}{\ensuremath{\left<p_\mathrm{T}\right>}}

\newcommand{\yLAB}{\ensuremath{y_\mathrm{LAB}}}
\newcommand{\yNN}{\ensuremath{y_\mathrm{NN}}}
\newcommand{\ystar}{\ensuremath{y^*}}

\newcommand{\pTjet}{\ensuremath{p_{\mathrm{T,jet}}}}
\newcommand{\pTjetch}{\ensuremath{p_\mathrm{T,jet}^\mathrm{ch}}}
\newcommand{\pTjetchemb}{\ensuremath{p_\mathrm{T,jet}^\mathrm{ch,emb}}}
\newcommand{\pTtrig}{\ensuremath{p_{\mathrm{T,trig}}}}
\newcommand{\pTassoc}{\ensuremath{p_{\mathrm{T,assoc}}}}
\newcommand{\pTtrk}{\ensuremath{p_{\mathrm{T,trk}}}}
\newcommand{\pTemb}{\ensuremath{p_{\mathrm{T,emb}}}}

\newcommand{\pTjetpart}{\ensuremath{p_{\mathrm{T,jet}^\mathrm{part}}}}
\newcommand{\pTjetdet}{\ensuremath{p_{\mathrm{T,jet}^\mathrm{det}}}}

\newcommand{\pThadron}{\ensuremath{p_{\mathrm{T,hadron}}}}
\newcommand{\ET}{\ensuremath{E_{\mathrm T}}}

\newcommand{\dNdpT}{\ensuremath{\frac{\rm{d}N}{\mathrm{d} \pT}}}

\newcommand{\pizero}{\ensuremath{\pi^0}}
\newcommand{\kzerol}{\ensuremath{\mathrm{K}^{0}_\mathrm{L}}}
\newcommand{\kzeros}{\ensuremath{\mathrm{K}^{0}_\mathrm{S}}}

\newcommand{\zleading}{\ensuremath{z_\mathrm{leading}}}


\newcommand{\DCAxy}{\ensuremath{DCA_{\mathrm xy}}}
\newcommand{\sDCAxy}{\ensuremath{sDCA_{\mathrm xy}}}


\newcommand{\qhat}{\ensuremath{\hat{q}}}
\newcommand{\vtwo}{\ensuremath{v_2}}


\newcommand{\sigdab}{\ensuremath{\sigma_{\delta,ab}}}

\newcommand{\RAA}{\ensuremath{R_\mathrm{AA}}}
\newcommand{\RCP}{\ensuremath{R_\mathrm{CP}}}
\newcommand{\ICP}{\ensuremath{I_\mathrm{CP}}}
\newcommand{\IAA}{\ensuremath{I_{\rm{AA}}}}

\newcommand{\RpPb}{\ensuremath{R_\mathrm{pPb}}}
\newcommand{\QpPb}{\ensuremath{Q_\mathrm{pPb}}}

\newcommand{\Drecoil}{\ensuremath{\Delta_\mathrm{recoil}}}

\newcommand{\tg}{\ensuremath{\theta_{\mathrm{g}}}}
\newcommand{\rg}{\ensuremath{R_{\mathrm{g}}}}
\newcommand{\zg}{\ensuremath{z_{\mathrm{g}}}}
\newcommand{\pTsub}{\ensuremath{p_{\mathrm{T,subleading}}}}
\newcommand{\pTlead}{\ensuremath{p_{\mathrm{T,leading}}}}


\newcommand{\vzero}{\ensuremath{\mathrm{V0}}}
\newcommand{\vzeroA}{\ensuremath{\mathrm{V0A}}}
\newcommand{\vzeroC}{\ensuremath{\mathrm{V0C}}}
\newcommand{\vzeroM}{\ensuremath{\mathrm{V0M}}}
\newcommand{\vzeroAscaled}{\ensuremath{\mathrm{V0A}/\left<\mathrm{V0A}\right>}}
\newcommand{\vzeroCscaled}{\ensuremath{\mathrm{V0C}/\left<\mathrm{V0C}\right>}}
\newcommand{\vzeroMscaled}{\ensuremath{\mathrm{V0M}/\left<\mathrm{V0M}\right>}}


==> Chapter4/commands.tex <==

\newcommand{\pp}           {pp\xspace}
\newcommand{\ppbar}        {\mbox{$\mathrm {p\overline{p}}$}\xspace}
\newcommand{\XeXe}         {\mbox{Xe--Xe}\xspace}
\newcommand{\PbPb}         {\mbox{Pb--Pb}\xspace}
\newcommand{\pA}           {\mbox{pA}\xspace}
\newcommand{\pPb}          {\mbox{p--Pb}\xspace}
\newcommand{\Pbp}          {\mbox{Pb--p}\xspace}
\newcommand{\AuAu}         {\mbox{Au--Au}\xspace}
\newcommand{\dAu}          {\mbox{d--Au}\xspace}

\newcommand{\s}            {\ensuremath{\sqrt{s}}\xspace}
\newcommand{\snn}          {\ensuremath{\sqrt{s_{\mathrm{NN}}}}\xspace}
\newcommand{\pt}           {\ensuremath{p_{\rm T}}\xspace}
\newcommand{\meanpt}       {$\langle p_{\mathrm{T}}\rangle$\xspace}
\newcommand{\ycms}         {\ensuremath{y_{\rm CMS}}\xspace}
\newcommand{\ylab}         {\ensuremath{y_{\rm lab}}\xspace}
\newcommand{\etarange}[1]  {\mbox{$\left | \eta \right |~<~#1$}}
\newcommand{\yrange}[1]    {\mbox{$\left | y \right |~<~#1$}}
\newcommand{\dndy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\dndeta}       {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}\eta}\xspace}
\newcommand{\avdndeta}     {\ensuremath{\langle\dndeta\rangle}\xspace}
\newcommand{\dNdy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\Npart}        {\ensuremath{N_\mathrm{part}}\xspace}
\newcommand{\Ncoll}        {\ensuremath{N_\mathrm{coll}}\xspace}
\newcommand{\dEdx}         {\ensuremath{\textrm{d}E/\textrm{d}x}\xspace}
\newcommand{\RpPb}         {\ensuremath{R_{\rm pPb}}\xspace}

\newcommand{\nineH}        {$\sqrt{s}~=~0.9$~Te\kern-.1emV\xspace}
\newcommand{\seven}        {$\sqrt{s}~=~7$~Te\kern-.1emV\xspace}
\newcommand{\thirteen}     {$\sqrt{s}~=~13$~Te\kern-.1emV\xspace}
\newcommand{\twoH}         {$\sqrt{s}~=~0.2$~Te\kern-.1emV\xspace}
\newcommand{\twosevensix}  {$\sqrt{s}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\five}         {$\sqrt{s}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\twosevensixnn}{$\sqrt{s_{\mathrm{NN}}}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\fivenn}       {$\sqrt{s_{\mathrm{NN}}}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\fivennx}       {$\sqrt{s_{\mathrm{NN}}}~=~5.44$~Te\kern-.1emV\xspace}
\newcommand{\eightonesixnn}{$\sqrt{s_{\mathrm{NN}}}~=~8.16$~Te\kern-.1emV\xspace}
\newcommand{\LT}           {L{\'e}vy-Tsallis\xspace}
\newcommand{\GeVc}         {Ge\kern-.1emV/$c$\xspace}
\newcommand{\MeVc}         {Me\kern-.1emV/$c$\xspace}
\newcommand{\TeV}          {Te\kern-.1emV\xspace}
\newcommand{\GeV}          {Ge\kern-.1emV\xspace}
\newcommand{\MeV}          {Me\kern-.1emV\xspace}
\newcommand{\GeVmass}      {Ge\kern-.2emV/$c^2$\xspace}
\newcommand{\MeVmass}      {Me\kern-.2emV/$c^2$\xspace}
\newcommand{\lumi}         {\ensuremath{\mathcal{L}}\xspace}

\newcommand{\ITS}          {\rm{ITS}\xspace}
\newcommand{\TOF}          {\rm{TOF}\xspace}
\newcommand{\ZDC}          {\rm{ZDC}\xspace}
\newcommand{\ZDCs}         {\rm{ZDCs}\xspace}
\newcommand{\ZNA}          {\rm{ZNA}\xspace}
\newcommand{\ZNC}          {\rm{ZNC}\xspace}
\newcommand{\SPD}          {\rm{SPD}\xspace}
\newcommand{\SDD}          {\rm{SDD}\xspace}
\newcommand{\SSD}          {\rm{SSD}\xspace}
\newcommand{\TPC}          {\rm{TPC}\xspace}
\newcommand{\TRD}          {\rm{TRD}\xspace}
\newcommand{\VZERO}        {\rm{V0}\xspace}
\newcommand{\VZEROA}       {\rm{V0A}\xspace}
\newcommand{\VZEROC}       {\rm{V0C}\xspace}
\newcommand{\Vdecay} 	   {\ensuremath{V^{0}}\xspace}

\newcommand{\ee}           {\ensuremath{e^{+}e^{-}}} 
\newcommand{\pip}          {\ensuremath{\pi^{+}}\xspace}
\newcommand{\pim}          {\ensuremath{\pi^{-}}\xspace}
\newcommand{\kap}          {\ensuremath{\rm{K}^{+}}\xspace}
\newcommand{\kam}          {\ensuremath{\rm{K}^{-}}\xspace}
\newcommand{\pbar}         {\ensuremath{\rm\overline{p}}\xspace}
\newcommand{\kzero}        {\ensuremath{{\rm K}^{0}_{\rm{S}}}\xspace}
\newcommand{\lmb}          {\ensuremath{\Lambda}\xspace}
\newcommand{\almb}         {\ensuremath{\overline{\Lambda}}\xspace}
\newcommand{\Om}           {\ensuremath{\Omega^-}\xspace}
\newcommand{\Mo}           {\ensuremath{\overline{\Omega}^+}\xspace}
\newcommand{\X}            {\ensuremath{\Xi^-}\xspace}
\newcommand{\Ix}           {\ensuremath{\overline{\Xi}^+}\xspace}
\newcommand{\Xis}          {\ensuremath{\Xi^{\pm}}\xspace}
\newcommand{\Oms}          {\ensuremath{\Omega^{\pm}}\xspace}
\newcommand{\degree}       {\ensuremath{^{\rm o}}\xspace}

==> Chapter5/commands.tex <==

\newcommand{\pp}           {pp\xspace}
\newcommand{\ppbar}        {\mbox{$\mathrm {p\overline{p}}$}\xspace}
\newcommand{\XeXe}         {\mbox{Xe--Xe}\xspace}
\newcommand{\PbPb}         {\mbox{Pb--Pb}\xspace}
\newcommand{\pA}           {\mbox{pA}\xspace}
\newcommand{\pPb}          {\mbox{p--Pb}\xspace}
\newcommand{\AuAu}         {\mbox{Au--Au}\xspace}
\newcommand{\dAu}          {\mbox{d--Au}\xspace}

\newcommand{\s}            {\ensuremath{\sqrt{s}}\xspace}
\newcommand{\snn}          {\ensuremath{\sqrt{s_{\mathrm{NN}}}}\xspace}
\newcommand{\pt}           {\ensuremath{p_{\rm T}}\xspace}
\newcommand{\meanpt}       {$\langle p_{\mathrm{T}}\rangle$\xspace}
\newcommand{\ycms}         {\ensuremath{y_{\rm CMS}}\xspace}
\newcommand{\ylab}         {\ensuremath{y_{\rm lab}}\xspace}
\newcommand{\etarange}[1]  {\mbox{$\left | \eta \right |~<~#1$}}
\newcommand{\yrange}[1]    {\mbox{$\left | y \right |~<~#1$}}
\newcommand{\dndy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\dndeta}       {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}\eta}\xspace}
\newcommand{\dnchdeta}     {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}\eta}\xspace}
\newcommand{\avdndeta}     {\ensuremath{\langle\dndeta\rangle}\xspace}
\newcommand{\dNdy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\Npart}        {\ensuremath{N_\mathrm{part}}\xspace}
\newcommand{\Ncoll}        {\ensuremath{N_\mathrm{coll}}\xspace}
\newcommand{\dEdx}         {\ensuremath{\textrm{d}E/\textrm{d}x}\xspace}
\newcommand{\RpPb}         {\ensuremath{R_{\rm pPb}}\xspace}

\newcommand{\Tch}          {\ensuremath{T_{\rm chem}}\xspace}

\newcommand{\mt}           {\ensuremath{m_{\rm T}}\xspace}
\newcommand{\kt}           {\ensuremath{k_{\rm T}}\xspace}
\newcommand{\ks}           {\ensuremath{k^*}\xspace}
\newcommand{\rs}           {\ensuremath{r^*}\xspace}
\newcommand{\ck}           {\ensuremath{C(k^*)}\xspace}
\newcommand{\sr}           {\ensuremath{S(r^*)}\xspace}
\newcommand{\wf}           {\ensuremath{\psi(\vec{\rs},\vec{\ks})}\xspace}
\newcommand{\rc}           {\ensuremath{r_\mathrm{core}}\xspace}
\newcommand{\pP}           {\ensuremath{\mbox{p--p}}\xspace}
\newcommand{\ApAP}         {\ensuremath{\mbox{\pbar--\pbar}}\xspace}
\newcommand{\pL}           {\ensuremath{\mbox{p--\lmb}}\xspace}
\newcommand{\pK}           {\ensuremath{\mbox{p--}\mathrm{K}^-}\xspace}
\newcommand{\ApAL}         {\ensuremath{\mbox{\pbar--\almb}}\xspace}
\newcommand{\LL}           {\ensuremath{\mbox{\lmb--\lmb}}\xspace}
\newcommand{\pSo}          {\ensuremath{\mbox{p--\So}}\xspace}
\newcommand{\pXi}          {\ensuremath{\mbox{p--\X}}\xspace}
\newcommand{\pipi}          {\ensuremath{\uppi\mbox{--}\uppi}\xspace}
\newcommand{\kaka}          {\ensuremath{\mbox{K--K}}\xspace}
\newcommand{\HALQCD}{HAL QCD\xspace}
\newcommand{\pSiZero}{\ensuremath{\mbox{p--$\Sigma^0$}}~}

\newcommand{\pXim}{\ensuremath{\mbox{p--$\Xi^{-}$}}\xspace}
\newcommand{\pXip}{\ensuremath{\overline{\mathrm{p}}$\mbox{--}$\xip}\xspace}

\newcommand{\pOmbound}{\ensuremath{\mbox{p--$\Omega^{-}$}}\xspace}
\newcommand{\pOm}{\ensuremath{\mbox{p--$\Omega^{-}$}}\xspace}
\newcommand{\pOp}{\ensuremath{\overline{\mathrm{p}}$\mbox{--}$\omp}\xspace}
\newcommand{\pO}{\ensuremath{\mbox{p--$\Omega$}}\xspace}

\newcommand{\Kmp}{\ensuremath{\mathrm {K^-p}}\xspace}
\newcommand{\Kzn}{\ensuremath{\mathrm {\overline K^0n}}\xspace}
\newcommand{\CF}           {C(\ks)\xspace}

\newcommand{\siZ}          {\ensuremath{\upSigma^{0}}\xspace}
\newcommand{\siP}          {\ensuremath{\upSigma^{+}}\xspace}
\newcommand{\siM}          {\ensuremath{\upSigma^{-}}\xspace}
\newcommand{\asiZ}         {\ensuremath{\overline{\upSigma^{0}}}\xspace}
\newcommand{\psiZCF}       {\rm{p}\mbox{--}\siZ}
\newcommand{\SNCF}         {\rm{N}\mbox{--}\ensuremath{\upSigma}\xspace}
\newcommand{\LNCF}         {\rm{N}\mbox{--}\ensuremath{\upLambda}\xspace}
\newcommand{\apasiZCF}     {\ensuremath{\overline{\mathrm{p}}}\mbox{--}\asiZ}
\newcommand{\psiZCombCF}   {\rm{p}\mbox{--}\siZ \ensuremath{\oplus} \apasiZCF}
\newcommand{\SB}           {\ensuremath{(\upLambda\gamma)}\xspace}
\newcommand{\pSBCF}        {\rm{p}\mbox{--}\SB}

\newcommand{\pLCF}         {\rm{p}\mbox{--}\lmb}
\newcommand{\nSplusCF}     {\rm{n}\mbox{--}\ensuremath{\upSigma^{+}}}

\newcommand{\Ledn}         {Lednick\'y--Lyuboshits approach\xspace}
\newcommand{\chiEFT}       {\ensuremath{\chi}\rm{EFT}\xspace}
\newcommand{\fss}          {\rm{fss2}\xspace}
\newcommand{\ESC}          {\rm{ESC16}\xspace}
\newcommand{\NSC}          {\rm{NSC97f}\xspace}

\newcommand{\hyp}    {$^{3}_{\Lambda}\mathrm H$\xspace}
\newcommand{\antihyp}{$^{3}_{\bar{\Lambda}} \overline{\mathrm H}$\xspace}

\newcommand{\he}     {$^{3}\mathrm{He}$\xspace}
\newcommand{\antihe} {$^{3}\mathrm{\overline{He}}$\xspace}

\newcommand{\hefour}     {$^{4}\mathrm{He}$\xspace}
\newcommand{\antihefour} {$^{4}\mathrm{\overline{He}}$\xspace}


\newcommand{\tri}     {$^{3}\mathrm{H}$}
\newcommand{\antitri} {$^{3}\mathrm{\overline{H}}$}


\newcommand{\dedx}   {d$E$/d$x$}
\newcommand{\mom}    {\mbox{\rm MeV$\kern-0.15em /\kern-0.12em c$}}
\newcommand{\gmom}   {\mbox{\rm GeV$\kern-0.15em /\kern-0.12em c$}}
\newcommand{\mass}   {\mbox{\rm GeV$\kern-0.15em /\kern-0.12em c^2$}}
\newcommand{\Mmass}  {\mbox{\rm MeV$\kern-0.15em /\kern-0.12em c^2$}}
\newcommand{\Dp}     {$\Delta p_0$}
\newcommand{\Dr}     {$\Delta \rho_0$}

\newcommand{\vtwo}   {$v_{2}$\xspace}
\newcommand{\vthree} {$v_{3}$\xspace}

\newcommand{\nineH}        {$\sqrt{s}~=~0.9$~Te\kern-.1emV\xspace}
\newcommand{\seven}        {$\sqrt{s}~=~7$~Te\kern-.1emV\xspace}
\newcommand{\twoH}         {$\sqrt{s}~=~0.2$~Te\kern-.1emV\xspace}
\newcommand{\twosevensix}  {$\sqrt{s}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\five}         {$\sqrt{s}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\twosevensixnn}{$\sqrt{s_{\mathrm{NN}}}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\fivenn}       {$\sqrt{s_{\mathrm{NN}}}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\LT}           {L{\'e}vy-Tsallis\xspace}
\newcommand{\GeVc}         {Ge\kern-.1emV/$c$\xspace}
\newcommand{\MeVc}         {Me\kern-.1emV/$c$\xspace}
\newcommand{\TeV}          {Te\kern-.1emV\xspace}
\newcommand{\GeV}          {Ge\kern-.1emV\xspace}
\newcommand{\MeV}          {Me\kern-.1emV\xspace}
\newcommand{\GeVmass}      {Ge\kern-.2emV/$c^2$\xspace}
\newcommand{\MeVmass}      {Me\kern-.2emV/$c^2$\xspace}
\newcommand{\lumi}         {\ensuremath{\mathcal{L}}\xspace}

\newcommand{\ITS}          {\rm{ITS}\xspace}
\newcommand{\TOF}          {\rm{TOF}\xspace}
\newcommand{\ZDC}          {\rm{ZDC}\xspace}
\newcommand{\ZDCs}         {\rm{ZDCs}\xspace}
\newcommand{\ZNA}          {\rm{ZNA}\xspace}
\newcommand{\ZNC}          {\rm{ZNC}\xspace}
\newcommand{\SPD}          {\rm{SPD}\xspace}
\newcommand{\SDD}          {\rm{SDD}\xspace}
\newcommand{\SSD}          {\rm{SSD}\xspace}
\newcommand{\TPC}          {\rm{TPC}\xspace}
\newcommand{\TRD}          {\rm{TRD}\xspace}
\newcommand{\VZERO}        {\rm{V0}\xspace}
\newcommand{\VZEROA}       {\rm{V0A}\xspace}
\newcommand{\VZEROC}       {\rm{V0C}\xspace}
\newcommand{\Vdecay} 	   {\ensuremath{V^{0}}\xspace}

\newcommand{\ee}           {e$^{+}$e$^{-}$\xspace} 
\newcommand{\pip}          {\ensuremath{\pi^{+}}\xspace}
\newcommand{\pim}          {\ensuremath{\pi^{-}}\xspace}
\newcommand{\kap}          {\ensuremath{\rm{K}^{+}}\xspace}
\newcommand{\kam}          {\ensuremath{\rm{K}^{-}}\xspace}
\newcommand{\pbar}         {\ensuremath{\rm\overline{p}}\xspace}
\newcommand{\kzero}        {\ensuremath{{\rm K}^{0}_{\rm{S}}}\xspace}
\newcommand{\lmb}          {\ensuremath{\Lambda}\xspace}
\newcommand{\almb}         {\ensuremath{\overline{\Lambda}}\xspace}
\newcommand{\Om}           {\ensuremath{\Omega^-}\xspace}
\newcommand{\Mo}           {\ensuremath{\overline{\Omega}^+}\xspace}
\newcommand{\X}            {\ensuremath{\Xi^-}\xspace}
\newcommand{\Ix}           {\ensuremath{\overline{\Xi}^+}\xspace}
\newcommand{\Xis}          {\ensuremath{\Xi^{\pm}}\xspace}
\newcommand{\Oms}          {\ensuremath{\Omega^{\pm}}\xspace}
\newcommand{\degree}       {\ensuremath{^{\rm o}}\xspace}

==> Chapter6/aliceCDSpreprint_ScientificNotationCommands.tex <==





\newcommand {\stat}     {({\it stat.})~}
\newcommand {\syst}     {({\it syst.})~}

\newcommand{\ie}        {$i.e.$~}
\newcommand{\eg}        {$e.g.$~}
\newcommand{\Eg}        {$E.g.$~}
\newcommand{\Fig}       {\textsc{f}ig.~}
\newcommand{\fig}       {\Fig}
\newcommand{\Figs}      {\textsc{f}igs.~}
\newcommand{\figs}      {\Figs}
\newcommand{\Figure}    {\textsc{f}igure~}
\newcommand{\Figures}   {\textsc{f}igures~}
\newcommand{\Tab}       {\textsc{t}ab.~}
\newcommand{\tab}       {\Tab}
\newcommand{\Table}     {\textsc{t}able~}
\newcommand{\Tables}    {\textsc{t}ables~}
\newcommand{\chap}      {\textsc{c}hap.~}
\newcommand{\parag}     {\textsc{p}ar.~}
\newcommand{\appdx}     {\textsc{a}pp.~}
\newcommand{\eq}        {\textsc{e}q.~}
\newcommand{\opt}        {\textsc{o}pt.~}

\newcommand{\tune}      {\emph{tune}}
\newcommand{\tunes}     {\emph{tunes}\xspace}


\newcommand{\orderOf}[1]{\ensuremath{\mathcal{O}}(#1)}

\newcommand{\CheckGr}   {\textcolor{Green}{\normalsize \CheckmarkBold}} 
\newcommand{\SurpriseGr}{\textcolor{Green}{\textbf{!}{\scriptsize !}}}
\newcommand{\Wtf}       {\textcolor{IndianRed}{\textbf{?}!}}
\newcommand{\NB}        {\textcolor{IndianRed}{\HandRight}}
\newcommand{\Caution}   {\textcolor{IndianRed}{\scriptsize \textlhdbend}}
\newcommand{\NoWay}     {\textcolor{IndianRed}{\normalsize \XSolidBrush}}
\newcommand{\UnderWork} {\textcolor{Blue}{\Large \dsagricultural}}
\newcommand{\ToDo}      {\textcolor{Gray}{\scriptsize \textsc{ToDo}}}




\newcommand {\pT}           {\ensuremath{p_{\rm T}}}
\newcommand {\pTlw}         {\ensuremath{p_{\rm T}^{lw} }}
\newcommand {\pTIdx}[1]     {\ensuremath{p_{\text{\textsc{t},#1}}}}
\newcommand {\pTExp}[1]     {\ensuremath{p_{\text{\textsc{t}}}^{#1}}}
\newcommand {\pTIdxExp}[2]  {\ensuremath{p_{\text{\textsc{t},#1}}^{#2}}}
\newcommand {\pTof}[1]      {\ensuremath{p_{\text{\textsc{t}}} \text{(#1)}}}
\newcommand {\pTchJet}      {\ensuremath{p_{\text{\textsc{t},jet}}^{\text{ch}}}}
\newcommand {\pTchEmJet}    {\ensuremath{p_{\text{\textsc{t},jet}}^{\text{ch+em}}}}
\newcommand {\meanpT}       {\ensuremath{\langle p_{\textsc{t}} \kern-0.1em\rangle}}
\newcommand {\mean}[1]      {\ensuremath{\langle #1 \kern-0.1em\rangle}} 
\newcommand {\sqrtSnn}      {\ensuremath{\sqrt{s_\text{\textsc{nn}}}}}
\newcommand {\sqrtS}        {\ensuremath{\sqrt{s}}}
\newcommand {\vTwo}         {\ensuremath{v_{\text{2}}}}
\newcommand {\vThree}       {\ensuremath{v_{\text{3}}}}
\newcommand {\vFour}        {\ensuremath{v_{\text{4}}}}
\newcommand {\vFive}        {\ensuremath{v_{\text{5}}}}
\newcommand {\vSix}         {\ensuremath{v_{\text{6}}}}
\newcommand {\vN}           {\ensuremath{v_{\text{n}}}}
\newcommand {\eT}           {\ensuremath{E_{\text{\textsc{t}}}}}
\newcommand {\mT}           {\ensuremath{m_{\text{\textsc{t}}}}}
\newcommand {\mTmZero}      {\ensuremath{m_{\text{\textsc{t}}} - m_0}}
\newcommand {\minv}         {\mbox{$m_{\ee}$}}
\newcommand {\rap}          {\mbox{$y$}}
\newcommand {\rapLab}       {\mbox{$y_{\text{lab}}$}}
\newcommand {\rapCms}       {\mbox{$y_{\text{\textsc{cms} }}$}}
\newcommand {\absrap}       {\mbox{$\left | y \right | $}}
\newcommand {\rapPart}[1]   {\mbox{$\left | y\text{(#1)} \right | $}}
\newcommand {\rapXi}        {\mbox{$\left | y(\rmXi) \right | $}}
\newcommand {\rapJpsi}      {\mbox{$y_{\tiny \rmJpsi}$}}
\newcommand {\abspseudorap} {\mbox{$\left | \eta \right | $}}
\newcommand {\pseudorap}    {\mbox{$\eta$}}
\newcommand {\pseudorapLab} {\mbox{$\eta_{\,\text{lab}}$}}
\newcommand {\pseudorapCms} {\mbox{$\eta_{\text{\textsc{cms} }}$}}
\newcommand {\cTau}         {\ensuremath{c.\tau}}
\newcommand {\sigee}        {$\sigma_E$/$E$}
\newcommand {\AxEff}        {\ensuremath{\mathscr{A}.\varepsilon}}


\newcommand{\dd}{\mathop{}\!\mathrm{d}}
\newcommand {\oneOverpipT}  {\ensuremath{1/2\pi\pT}}
\newcommand {\crossSec}[1]  {\mbox{$\sigma_{\scriptsize \rm #1}$}}
\newcommand {\visCrossSec}[1]  {\mbox{$\sigma_{\scriptsize \rm #1}^{visible}$}}
\newcommand {\dsigmady}     {\ensuremath{\mathrm{d}\sigma/\mathrm{d}y}}
\newcommand {\dsigmadpt}    {\ensuremath{\mathrm{d}^{2}\sigma/\mathrm{d}\pT}}
\newcommand {\dsigmadptdy}  {\ensuremath{\mathrm{d}^{2}\sigma/\mathrm{d}\pT\mathrm{d}y}}
\newcommand {\dsigmadptdeta}{\ensuremath{\mathrm{d}^{2}\sigma/\mathrm{d}\pT\mathrm{d}\eta}}
\newcommand {\dsigmaXdy}[1] {\ensuremath{\mathrm{d}\sigma\text{(#1)}/\mathrm{d}y}}
\newcommand {\dsigmaXdpt}[1]{\ensuremath{\mathrm{d}\sigma\text{(#1)}/\mathrm{d}\pT}}
\newcommand {\dsigmaXdptdy}[1]  {\ensuremath{\mathrm{d}^{2}\sigma\text{(#1)}/\mathrm{d}\pT\mathrm{d}y}}
\newcommand {\dNdy}         {\ensuremath{\mathrm{d}N/\mathrm{d}y}}
\newcommand {\dNXdy}[1]     {\ensuremath{\mathrm{d}N\text{(#1)}/\mathrm{d}y}}
\newcommand {\dNJpsidy}     {\dNXdy{\rmJpsi}}
\newcommand {\dNdpt}        {\ensuremath{\mathrm{d}N/\mathrm{d}\pT }}
\newcommand {\dNXdptdy}[1]  {\ensuremath{\mathrm{d}^{2}N\text{(#1)}/\mathrm{d}\pT\mathrm{d}y}}
\newcommand {\dNdptdy}      {\ensuremath{\mathrm{d}^{2}N/\mathrm{d}\pT\mathrm{d}y }}
\newcommand {\dNdptdeta}    {\ensuremath{\mathrm{d}^{2}N/\mathrm{d}\pT\mathrm{d}\eta }}
\newcommand {\fracdsigmadptdy}  {\ensuremath{ \frac{\mathrm{d}^{2}\sigma}{\mathrm{d}\pT\mathrm{d}y}}}
\newcommand {\fracdNdptdy}  {\ensuremath{ \frac{\mathrm{d}^{2}N}{\mathrm{d}\pT\mathrm{d}y } }}
\newcommand {\fracdNdy}     {\ensuremath{ \frac{\dN}{\dy}}}
\newcommand {\fracdNdyBold} {\ensuremath{ \frac{\bm{\dN}}{\bm{\dy}}}}

\newcommand {\dNdmtdy}      {\ensuremath{\mathrm{d}^{2}N/\mathrm{d}\mT\mathrm{d}y }}
\newcommand {\dN}           {\ensuremath{\mathrm{d}N }}
\newcommand {\Npp}          {\ensuremath{N_{\textsc{\pp}}}}
\newcommand {\dNsquared}    {\ensuremath{\mathrm{d}^{2}N }}
\newcommand {\dsquared}     {\ensuremath{\mathrm{d}^{2} }}
\newcommand {\dpT}          {\ensuremath{\mathrm{d}\pT }}
\newcommand {\dy}           {\ensuremath{\mathrm{d}y}}
\newcommand {\dNdyBold}     {\ensuremath{\bm{\dN/\dy}}}
\newcommand {\dNchdy}       {\ensuremath{\mathrm{d}N_\text{ch}/\mathrm{d}y }}
\newcommand {\dNchdeta}     {\ensuremath{\mathrm{d}N_\text{ch}/\mathrm{d}\eta }}
\newcommand {\dNchdptdeta}  {\ensuremath{\mathrm{d}^{2}N_\text{ch}/\mathrm{d}\pT\mathrm{d}\eta }}
\newcommand {\RAA}          {\ensuremath{R_\text{AA}}}
\newcommand {\RpA}          {\ensuremath{R_\text{pA}}}
\newcommand {\RpPb}         {\ensuremath{R_\text{pPb}}}
\newcommand {\RPbp}         {\ensuremath{R_\text{Pbp}}}
\newcommand {\RAuAu}        {\ensuremath{R_\text{AuAu}}}
\newcommand {\RPbPb}        {\ensuremath{R_\text{PbPb}}}
\newcommand {\Rcp}          {\ensuremath{R_\text{CP}}}
\newcommand {\hPMVzsCorrel} {\ensuremath{(\text{\hPM-V0})}}
\newcommand {\hVzsCorrel}   {\ensuremath{(\text{h-V0})}}
\newcommand {\mPDG}[1]      {\ensuremath{m_{\text{pdg}}(#1)}}



\newcommand {\Nevt}         {\ensuremath{N_\text{evt}}}
\newcommand {\NevtINEL}     {\ensuremath{N_\text{evt}(\textsc{inel})}}
\newcommand {\NevtNSD}      {\ensuremath{N_\text{evt}(\textsc{nsd})}}
\newcommand {\INEL}         {\ensuremath{\textsc{inel}}}
\newcommand {\INELZero}     {\ensuremath{\textsc{inel}>0}}
\newcommand {\NSD}          {\ensuremath{\textsc{nsd}}}
\newcommand {\dEdx}         {\ensuremath{\textup{d}E/\textup{d}x }}

\newcommand {\bsTe}      {\ensuremath{\bm{T_e}}}
\newcommand {\bsTb}      {\ensuremath{\bm{T_b}}}
\newcommand {\bsTt}      {\ensuremath{\bm{T_T}}}
\newcommand {\bsCt}      {\ensuremath{\bm{C_T}}}
\newcommand {\bsNt}      {\ensuremath{\bm{n}}}
\newcommand {\bsQt}      {\ensuremath{\bm{q}}}
\newcommand {\bsVt}      {\ensuremath{\bm{V}}}
\newcommand {\bsgVt}     {\ensuremath{\bm{g.V}}}
\newcommand {\bsNb}      {\ensuremath{\bm{n}}}
\newcommand {\bsFp}      {\ensuremath{\bm{f_P}}}
\newcommand {\bsCp}      {\ensuremath{\bm{C_P}}}

\newcommand {\Lint}         {\ensuremath{L_{\text{int}}}}

\newcommand {\rphi}         {\mbox{\ensuremath{(r,\varphi)}}}
\newcommand {\alphaS}       {\ensuremath{ \alpha_s}}
\newcommand {\chLeptonAsymm}{\ensuremath{ A_{\ell\ell} }}

\newcommand {\MeanNpart}    {\mbox{\ensuremath{\langle\kern-0.05em N_{part} \kern-0.05em \rangle}}}
\newcommand {\MeanNcoll}    {\mbox{\ensuremath{\langle\kern-0.05em N_{coll} \kern-0.05em \rangle}}}
\newcommand {\sigmaBarlow}  {\ensuremath{\sigma_{Barlow}}}
\newcommand {\sigmaStat}    {\ensuremath{\sigma_{stat}}}
\newcommand {\sigmaSyst}    {\ensuremath{\sigma_{syst}}}
\newcommand {\sigmaTot}     {\ensuremath{\sqrt{\sigmaStat^2 + \sigmaSyst^2}}}

\newcommand {\xXzero}     {\ensuremath{\textsc{x}/X_0}}



\newcommand {\eX}    {\ensuremath{\vec{e}_{\textsc{x}}}}
\newcommand {\eY}    {\ensuremath{\vec{e}_{\textsc{y}}}}
\newcommand {\eZ}    {\ensuremath{\vec{e}_{\textsc{z}}}}

\newcommand {\ePhi}  {\ensuremath{\vec{e}_{\varphi}}}
\newcommand {\eR}    {\ensuremath{\vec{e}_{r}}}



\newcommand{\Sherpa}        {\textsc{Sherpa}\xspace}
\newcommand{\Herwig}        {\textsc{Herwig++}\xspace}
\newcommand{\Epos}          {\textsc{Epos}\xspace}
\newcommand{\Pythia}        {\textsc{Pythia}\xspace}
\newcommand{\Pythiaeight}   {\Pythia~8\xspace}
\newcommand{\Rivet}         {\textsc{Rivet}\xspace}
\newcommand{\HepMC}         {\textsc{HepMc}\xspace}

\newcommand{\Root}          {\textsc{Root}\xspace}
\newcommand{\GeantFour}     {\textsc{Geant4}\xspace}
\newcommand{\Fluka}         {\textsc{Fluka}\xspace}


\newcommand {\pp}        {\ensuremath{\mbox{\text {p\kern-0.05em p}}}\xspace}
\newcommand {\rmpp}      {\ensuremath{\text{p\kern-0.05em p} }}
\newcommand {\ppbar}     {\mbox{$\text{p}\overline{\text{p}}$}}
\newcommand {\PbPb}      {\ensuremath{\mbox{\text{Pb--Pb}} }}
\newcommand {\rmPbPb}    {\ensuremath{\text{PbPb} }}
\newcommand {\AuAu}      {\ensuremath{\mbox{\text{Au--Au}} }}
\newcommand {\ArAr}      {\ensuremath{\mbox{\text{Ar--Ar}} }}
\newcommand {\CuCu}      {\ensuremath{\mbox{\text{Cu--Cu}} }}
\newcommand {\UU}        {\ensuremath{\mbox{\text{U--U}}   }}
\newcommand {\XeXe}      {\ensuremath{\mbox{\text{Xe--Xe}} }}
\renewcommand {\AA}      {\ensuremath{\text{A--A}          }} %
\newcommand {\rmAA}      {\ensuremath{\text{AA}            }} %
\newcommand {\pA}        {\ensuremath{\mbox{\text{p--A}}   }}
\newcommand {\rmpA}      {\ensuremath{\text{pA}            }} %
\newcommand {\dA}        {\ensuremath{\mbox{\text{d--A}}   }}
\newcommand {\pPb}       {\ensuremath{\mbox{\text{p--Pb}}  }}
\newcommand {\Pbp}       {\ensuremath{\mbox{\text{Pb--p}}  }}
\newcommand {\dAu}       {\ensuremath{\mbox{\text{d--Au}}  }}
\newcommand {\pAu}       {\ensuremath{\mbox{\text{p--Au}}  }}
\newcommand {\EplusEminus}      {\ee}
\newcommand {\ee}               {\mbox{$\text{e}^+\text{e}^-$}}
\newcommand {\Eplus}            {\mbox{$\text{e}^+$}}
\newcommand {\Eminus}           {\mbox{$\text{e}^-$}}
\newcommand {\MuPlusMuMinus}    {\mbox{$\mu^+\mu^-$}}
\newcommand {\MuPlus}           {\mbox{$\mu^+$}}
\newcommand {\MuMinus}          {\mbox{$\mu^-$}}


\newcommand {\massStyle}[1] {\mbox{\ensuremath{\text{#1}\kern-0.1em /\kern-0.12em c^2}}}
\newcommand {\mass}     {\massStyle{MeV}}
\newcommand {\kmass}    {\massStyle{keV}}
\newcommand {\mmass}    {\massStyle{MeV}}
\newcommand {\gmass}    {\massStyle{GeV}}

\newcommand {\unitStyle}[1] {\mbox{\ensuremath{\text{#1}}}}
\newcommand {\tev}      {\unitStyle{TeV}}
\newcommand {\gev}      {\unitStyle{GeV}}
\newcommand {\mev}      {\unitStyle{MeV}}
\newcommand {\kev}      {\unitStyle{keV}}
\newcommand {\J}        {\unitStyle{J}}

\newcommand {\momStyle}[1] {\mbox{\ensuremath{\text{#1}\kern-0.1em /\kern-0.12em c}}}
\newcommand {\mmom}     {\momStyle{MeV}}
\newcommand {\gmom}     {\momStyle{GeV}}

\newcommand {\fsec}       {\unitStyle{fs}}
\newcommand {\psec}       {\unitStyle{ps}}
\newcommand {\nsec}       {\unitStyle{ns}}
\newcommand {\musec}      {\mbox{$\mu\unitStyle{s}$}}
\newcommand {\millisec}   {\unitStyle{ms}}
\newcommand {\second}     {\unitStyle{s}}

\newcommand {\MHz}     {\unitStyle{MHz}}
\newcommand {\kHz}     {\unitStyle{kHz}}

\newcommand {\fmC}      {\mbox{$\unitStyle{fm}/\kern-0.12em c$}}

\newcommand {\fm}       {\unitStyle{fm}}
\newcommand {\nm}       {\unitStyle{nm}}
\newcommand {\mum}      {\mbox{$\mu\unitStyle{m}$}}
\newcommand {\mm}       {\unitStyle{mm}}
\newcommand {\cm}       {\unitStyle{cm}}
\newcommand {\m}        {\unitStyle{m}}

\newcommand {\cmq}      {\mbox{$\cm^2$}}
\newcommand {\mmq}      {\mbox{$\mm^2$}}
\newcommand {\mumq}     {\mbox{$\mum^2$}}

\newcommand {\fmCube}   {\mbox{\unitStyle{fm}$^3$}}

\newcommand {\mug}      {\mbox{$\mu\unitStyle{g}$}}
\newcommand {\mg}       {\unitStyle{mg}}
\newcommand {\gram}     {\unitStyle{g}}
\newcommand {\kg}       {\unitStyle{kg}}

\newcommand {\dens}     {\mbox{$\unitStyle{g}/\unitStyle{cm}^{3}$}}

\newcommand {\dg}       {\mbox{$\kern+0.1em ^\circ$}}


\newcommand {\lumi}     {\mbox{$\cm^{-2}\second^{-1}$}}

\newcommand {\barn}     {\unitStyle{b}}
\newcommand {\fb}       {\unitStyle{fb}}
\newcommand {\pb}       {\unitStyle{pb}}
\newcommand {\nb}       {\unitStyle{nb}}
\newcommand {\mub}      {\mbox{$\mu\unitStyle{b}$}}
\newcommand {\mb}       {\unitStyle{mb}}
\newcommand {\kb}       {\unitStyle{kb}}

\newcommand {\invmub}   {\mbox{$\mub^{-1}$}}
\newcommand {\invnb}    {\mbox{$\nb^{-1}$}}
\newcommand {\invpb}    {\mbox{$\pb^{-1}$}}
\newcommand {\invfb}    {\mbox{$\fb^{-1}$}}





\newcommand{\hPM}           {\ensuremath{h^{\pm}}}
\newcommand{\ePlusMinus}    {\mbox{$\mathrm {e^{\pm}}$}}
\newcommand{\muPlusMinus}   {\mbox{$\mathrm {\mu^{\pm}}$}}

\newcommand{\piZero}        {\mbox{$\mathrm {\pi^0}$}}
\newcommand{\piMinus}       {\mbox{$\mathrm {\pi^-}$}}
\newcommand{\piPlus}        {\mbox{$\mathrm {\pi^+}$}}
\newcommand{\piPlusMinus}   {\mbox{$\mathrm {\pi^{\pm}}$}}
\newcommand{\rmPiPlusMinus} {\piPlusMinus}
\newcommand{\rmPiPM}        {\piPlusMinus}
\newcommand{\rmPiMinus}     {\piMinus}
\newcommand{\rmPiPlus}      {\piPlus}

\newcommand{\Kzs}        {\mbox{$\mathrm {K^0_S}$}}
\newcommand{\rmKzero}    {\Kzs}
\newcommand{\Kzl}        {\mbox{$\mathrm {K^0_L}$}}
\newcommand{\rmKzeroL}   {\Kzl}
\newcommand{\Kminus}     {\mbox{$\mathrm {K^-}$}}
\newcommand{\rmKminus}   {\Kminus}
\newcommand{\Kplus}      {\mbox{$\mathrm {K^+}$}}
\newcommand{\rmKplus}    {\Kplus}
\newcommand{\Kplusmin}   {\mbox{$\mathrm {K^{\pm}}$}}
\newcommand{\rmKpm}      {\Kplusmin}
\newcommand{\rmKstar}    {\mbox{$\mathrm{K}^*\mathrm{(892)}^0$}}
\newcommand{\rmPhiMes}   {\mbox{$\mathrm {\phi(1020)}$}}

\newcommand{\proton}    {\mbox{$\mathrm {p}$}}
\newcommand{\pbar}      {\mbox{$\mathrm {\overline{p}}$}}
\newcommand{\pOrPbar}   {\mbox{$\mathrm {p^{\pm}}$}}


\newcommand{\rmLambdaZ}         {\mbox{$\mathrm {\Lambda}$}}
\newcommand{\rmAlambdaZ}        {\mbox{$\mathrm {\overline{\Lambda}}$}}
\newcommand{\rmLambda}          {\mbox{$\mathrm {\Lambda}$}}
\newcommand{\rmAlambda}         {\mbox{$\mathrm {\overline{\Lambda}}$}}
\newcommand{\rmLambdas}         {\mbox{$\mathrm {\Lambda \kern-0.2em + \kern-0.2em \overline{\Lambda}}$}}
\newcommand{\ratioLamOverKzs}   {\rmLambda/\rmKzero}

\newcommand{\rmSigma}       {\mbox{$\mathrm {\Sigma}$}}
\newcommand{\rmSigmaM}      {\mbox{$\mathrm{\Sigma}^{-}$}}
\newcommand{\rmSigmaP}      {\mbox{$\mathrm{\Sigma}^{+}$}}
\newcommand{\rmSigmaZero}   {\mbox{$\mathrm{\Sigma}^{0}$}}
\newcommand{\rmSigmaMres}   {\mbox{$\mathrm{\Sigma(1385)}^{-}$}}
\newcommand{\rmSigmaPres}   {\mbox{$\mathrm{\Sigma(1385)}^{+}$}}


\newcommand{\rmXi}      {\mbox{$\mathrm{\Xi}$}}
\newcommand{\rmXiM}     {\mbox{$\mathrm{\Xi}^{-}$}}
\newcommand{\rmXiPM}    {\mbox{$\mathrm {\Xi^{\pm}}$}}





\newcommand{\rmAxiP}    {\mbox{$\mathrm {\overline{\Xi}^{+}}$}}
\newcommand{\rmXis}     {\mbox{$\mathrm {\Xi^{-} \kern-0.3em + \kern-0.1em \overline{\Xi}^{+}}$}}
\newcommand{\rmXiZero}  {\mbox{$\mathrm {\Xi^{0}}$}}
\newcommand{\rmXiZ}     {\rmXiZero}
\newcommand{\rmXiZres}  {\mbox{$\mathrm {\Xi (1530)^{0}}$}}
\newcommand{\rmAxiZres} {\mbox{$\mathrm {\overline{\Xi} (1530)^{0}}$}}
\newcommand{\rmXiMres}  {\mbox{$\mathrm {\Xi (1530)^{-}}$}}
\newcommand{\rmAxiPres} {\mbox{$\mathrm {\overline{\Xi}(1530)^{+}}$}}

\newcommand{\rmOmega}   {\mbox{$\mathrm {\Omega}$}}
\newcommand{\rmOmegaM}  {\mbox{$\mathrm {\Omega^{-}}$}}
\newcommand{\rmAomegaP} {\mbox{$\mathrm {\overline{\Omega}^{+}}$}}
\newcommand{\rmOmegas}  {\mbox{$\mathrm {\Omega^{-} \kern-0.3em +  \kern-0.1em \overline{\Omega}^{+}}$}}
\newcommand{\rmOmegaPM} {\mbox{$\mathrm {\Omega^{\pm}}$}} 


\newcommand{\rmDeuton}   {\mbox{$\mathrm {d}$}}
\newcommand{\rmDeutonPM} {\mbox{$\mathrm {d}^{\pm}$}}
\newcommand{\rmTriton}   {\mbox{$\mathrm {t}$}}
\newcommand{\rmTritonPM} {\mbox{$\mathrm {t}^{\pm}$}}
\newcommand{\rmHeThree}  {\mbox{$\mathrm {^3He}$}}
\newcommand{\rmHeThreePM}{\mbox{$\mathrm {^3He^{2\pm}}$}}
\newcommand{\rmHeFour}   {\mbox{$\mathrm {^4He}$}}
\newcommand{\rmHeFourPM} {\mbox{$\mathrm {^4He^{2\pm}}$}}

\newcommand{\rmHypertriton}  {\mbox{$^{3}_{\Lambda}\mathrm{H}$}}


\newcommand{\rmJpsi}    {\mbox{$\mathrm{J\kern-0.05em /\kern-0.05em\psi}$}}
\newcommand{\rmPsiTwoS} {\mbox{$\mathrm {\psi(2S)}$}}
\newcommand{\rmChicZero}{\mbox{$\mathrm {\chi_{c_0}}$}}
\newcommand{\rmChicOne} {\mbox{$\mathrm {\chi_{c_1}}$}}
\newcommand{\rmChicTwo} {\mbox{$\mathrm {\chi_{c_2}}$}}
\newcommand{\rmChicJ}   {\mbox{$\mathrm {\chi_{c_J}}$}}

\newcommand{\rmLambdaC}         {\mbox{$\mathrm {\Lambda}_{c}^{+}$}}
\newcommand{\rmXiCplus}         {\mbox{$\mathrm {\Xi}_{c}^{+}$}}
\newcommand{\rmXiCzero}         {\mbox{$\mathrm {\Xi}_{c}^{0}$}}
\newcommand{\rmOmegaCzero}      {\mbox{$\mathrm {\Omega}_{c}^{0}$}}
\newcommand{\rmXiCCtwoPlus}     {\mbox{$\mathrm {\Xi}_{cc}^{2+}$}}
\newcommand{\rmOmegaCCtwoPlus}  {\mbox{$\mathrm {\Omega}_{ccc}^{2+}$}}


\newcommand{\rmDzero}   {\mbox{$\mathrm {D}^{0}$}}
\newcommand{\rmDzeroBar}{\mbox{$\mathrm {\overline{D}}^{0}$}}
\newcommand{\rmDplus}   {\mbox{$\mathrm {D}^{+}$}}
\newcommand{\rmDminus}  {\mbox{$\mathrm {D}^{+}$}}
\newcommand{\rmDpm}     {\mbox{$\mathrm {D}^{\pm}$}}
\newcommand{\rmDstar}   {\mbox{$\mathrm{D}^*\mathrm{(2010)}^+$}}
\newcommand{\rmDs}      {\mbox{$\mathrm {D}^{+}_{s}$}}

\newcommand{\rmBzero}       {\mbox{$\mathrm {B^{0}}$}}
\newcommand{\rmBplus}       {\mbox{$\mathrm {B^{+}}$}}
\newcommand{\rmBminus}      {\mbox{$\mathrm {B^{-}}$}}
\newcommand{\rmBplusMinus}  {\mbox{$\mathrm {B^{\pm}}$}}
\newcommand{\rmBzeroS}      {\mbox{$\mathrm {B^{0}_s}$}}


\newcommand{\rmUpsOneS}         {\mbox{$\mathrm {\Upsilon(1S)}$}}
\newcommand{\rmUpsTwoS}         {\mbox{$\mathrm {\Upsilon(2S)}$}}
\newcommand{\rmUpsThreeS}       {\mbox{$\mathrm {\Upsilon(3S)}$}}
\newcommand{\rmUpsTwoThreeS}    {\mbox{$\mathrm {\Upsilon(2S,3S)}$}}
\newcommand{\rmUpsnS}           {\mbox{$\mathrm {\Upsilon(nS)}$}}
\newcommand{\rmUpsOneTwoThreeS} {\mbox{$\mathrm {\Upsilon(1S,2S,3S)}$}}

\newcommand{\rmPhoton}      {\mbox{$\mathrm {\gamma}$}}
\newcommand{\rmWplus}       {\mbox{$\mathrm {W^{+}}$}}
\newcommand{\rmWminus}      {\mbox{$\mathrm {W^{-}}$}}
\newcommand{\rmWPlusMinus}  {\mbox{$\mathrm {W^{\pm}}$}}
\newcommand{\rmZzero}       {\mbox{$\mathrm {Z}$}}



\newcommand{\qqbar}             {\mbox{$\mathrm {q\overline{q}}$}}
\newcommand{\ccbar}             {\mbox{$\mathrm {c\overline{c}}$}}
\newcommand{\bbbar}             {\mbox{$\mathrm {b\overline{b}}$}}
\newcommand{\DDbar}             {\mbox{$\mathrm {D\overline{D}}$}}



